Challenges for modelling and analysis in embedded systems and systems-of-systems design

Over the last decade we have witnessed an increasing use of data processing in embedded systems. Where in the past the data processing was limited (if present at all) to the handling of a small number of "on-off control signals", more recently much more complex sensory data is being captured, processed and used to improve system performance and dependability. The advent of systems-of-systems aggravates the use of more and more data, for instance, by bringing together data from several independent sources, allowing, in principle, for even better performing systems. However, this ever stronger data-orientation brings along several challenges in system design, both technically and organisationally, and also forces manufacturers to think beyond their traditional field of expertise. In this short paper, I will address these new design challenges, through a number of examples. The paper finishes with concrete challenges for supporting tools and techniques for system design in this new context.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{Larsen, Legay, Nyman (Eds.): 1st Workshop on \\
Advances in Systems of Systems (AiSoS 2013)\\
EPTCS 133, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.133.5}{10.4204/EPTCS.133.5}}

